Chinese Spelling Error Detection Using a Fusion Lattice LSTM

Spelling error detection serves as a crucial preprocessing in many natural language processing applications. Due to the characteristics of Chinese Language, Chinese spelling error detection is more challenging than error detection in English. Existing methods are mainly under a pipeline framework, which artificially divides error detection process into two steps. Thus, these methods bring error propagation and cannot always work well due to the complexity of the language environment. Besides existing methods only adopt character or word information, and ignore the positive effect of fusing character, word, pinyin1 information together. We propose an LF-LSTM-CRF model, which is an extension of the LSTMCRF with word lattices and character-pinyin-fusion inputs. Our model takes advantage of the end-to-end framework to detect errors as a whole process, and dynamically integrates character, word and pinyin information. Experiments on the SIGHAN data show that our LF-LSTM-CRF outperforms existing methods with similar external resources consistently, and confirm the feasibility of adopting the end-to-end framework and the availability of integrating of character, word and pinyin information.

==> abstract.tex <==
\begin{abstract}
% Spelling error detection serves as a crucial preprocessing in many natural language processing applications. Due to the characteristics of Chinese Language, Chinese spelling error detection is more challenge than error detection in English. Existing methods are mainly under a pipeline framework, and artificially divide error detection process into two steps, which bring error propagation  and cannot always work well due to the complexity of the language environment. Besides existing methods only adopt character or word information, and ignore the positive  effect of fusing character, word, pinyin  information together. We propose a LSTM-CRF model with word lattices and  character and pinyin fusion inputs, called FL-LSTM-CRF, which  takes the advantage of the end to end framework to detect errors as a whole process, and dynamically integrates character, word and pinyin information for error detection. Experiments on the Sighan data shows our FL-LSTM-CRF consistently outperform existing methods with similar external resources, and prove the feasibility of adopting the end to end framework and the availability of integrating of character, word and pinyin information.


Spelling error detection serves as a crucial preprocessing in many natural language processing applications. Due to the characteristics of Chinese Language, Chinese spelling error detection is more challenging than error detection in English. Existing methods are mainly under a pipeline framework, which artificially divides error detection process into steps. Thus, these methods bring error propagation  and cannot always work well due to the complexity of the language environment. Besides existing methods only adopt character or word information, and ignore the positive  effect of fusing character, word and pinyin\footnote{pinyin is a system of writing Chinese in Latin characters which was introduced in China in the late 1950s. The term in Chinese means literally ‘spell-sound’} information together. We propose an
FL-LSTM-CRF model, which is an extension of the LSTM-CRF
with word lattices and character-pinyin-fusion inputs. Our model  takes  advantage of the end-to-end framework to detect errors as a whole process, and dynamically integrates character, word and pinyin information. Experiments on the SIGHAN data show that our FL-LSTM-CRF  outperforms existing methods with similar external resources consistently, and  confirm the feasibility of adopting the
end-to-end framework and the availability of integrating of
character, word and pinyin information.


% In addition, higher feasibility of adopting the end-to-end framework and  higher availability of integrating of character, word and pinyin information have been well proved by using our model.



% , and prove the feasibility of adopting the end-to-end framework and the availability of integrating of character, word and pinyin information.



%In English, every single word is directly typed by keyboard. 
%Unlike English, we have to use pinyin input method to type Chinese characters.
%By intuition, pinyin should be helpful in detecting spelling errors.
%In this paper, we propose the double lattice LSTM model to integrate character, word and pinyin features. 
%Firstly, for each input character sequence, we extract all word and pinyin subsequences 
%that matched from large automatically-obtained word and pinyin lexicon, respectively.
%Then we link characters with matched words or pinyin subsequences.
%Finally,  all information are feed to the double lattice LSTM model for error detection. 
%% Experiments show that pinyin is a discriminate feature and our model outperforms the baseline on the news dataset. 
%Experiments show that pinyin is a discriminate feature, 
%and our model integrates three features well and improves the detection performance. 
%% that the integration of three features, namely character, word and pinyin, 
%% is an effective way to improve the task performance, which proves the effectiveness and superiority of our model.
%Even limited by the amount of data size and data domain, our model obtains 
%a comparable performance on an out-domain SIGHAN bake-off dataset using a fine-tune method.
\end{abstract}
